A SSIM Guided cGAN Architecture For Clinically Driven Generative Image Synthesis of Multiplexed Spatial Proteomics Channels

Here we present a structural similarity index measure (SSIM) guided conditional Generative Adversarial Network (cGAN) that generatively performs image-to-image (i2i) synthesis to generate photo-accurate protein channels in multiplexed spatial proteomics images. This approach can be utilized to accurately generate missing spatial proteomics channels that were not included during experimental data collection either at the bench or the clinic. Experimental spatial proteomic data from the Human BioMolecular Atlas Program (HuBMAP) was used to generate spatial representations of missing proteins through a U-Net based image synthesis pipeline. HuBMAP channels were hierarchically clustered by the (SSIM) as a heuristic to obtain the minimal set needed to recapitulate the underlying biology represented by the spatial landscape of proteins. We subsequently prove that our SSIM based architecture allows for scaling of generative image synthesis to slides with up to 100 channels, which is better than current state of the art algorithms which are limited to data with 11 channels. We validate these claims by generating a new experimental spatial proteomics data set from human lung adenocarcinoma tissue sections and show that a model trained on HuBMAP can accurately synthesize channels from our new data set. The ability to recapitulate experimental data from sparsely stained multiplexed histological slides containing spatial proteomic will have tremendous impact on medical diagnostics and drug development, and also raises important questions on the medical ethics of utilizing data produced by generative image synthesis in the clinical setting. The algorithm that we present in this paper will allow researchers and clinicians to save time and costs in proteomics based histological staining while also increasing the amount of data that they can generate through their experiments.

==> sections/7_data.tex <==
\section{Data and Code Availability}
    For review, we have shared all code and new data generated. The new CODEX lung adenocarcioma dataset that we generated from human patients to validate the novel computational methods in this paper is available  \href{https://drive.google.com/drive/folders/10TC0JtX1IMmbZZN-i8NcUKTlyBd41429?usp=sharing}{here}. All of our code to recreate our results is available \href{https://github.com/aauthors131/multiplexed-image-synthesis}{here}. We also utilized previously published CODEX data from the HuBMAP consortium available  \href{https://portal.hubmapconsortium.org/search?entity_type\%5B0\%5D=Dataset}{here}. Specifically, we included the following HuBMAP samples in our training:\\
    
    HBM347.PSLC.425, HBM863.FDNH.844, HBM992.RHJW.288, HBM622.JXWQ.554, \\
    HBM495.VWBD.428, HBM857.ZBDC.975, HBM496.ZJFC.554, HBM465.HZHH.676, \\
    HBM887.SHVF.747, HBM268.NKXB.243, HBM938.TNNT.879, HBM597.KZXW.469, \\
    HBM373.LDGF.766, HBM522.BSZT.385, HBM528.NMQV.274, HBM396.BXSQ.568, \\
    HBM825.KFFT.669, HBM557.SGTC.262, HBM893.CCKX.496, HBM997.PVCF.629, \\
    HBM685.TBGN.663. 

==> sections/acknowledgement.tex <==
\section*{Acknowledgement}

    This work was supported by a University of Texas System Rising STARs Award (J.M.L) and the CPRIT First Time Faculty Award (J.M.L). All patient data collection was approved by IRB protocoal [REDACTED FOR ANONYMITY UNTIL CAMERA READY VERSION].


==> sections/authors.tex <==
% Enter the paper's authors in order
% \addauthor{Name}{email/homepage}{INSTITUTION_CODE}
\addauthor{Susan Student}{http://www.vision.inst.ac.uk/~ss}{1}
\addauthor{Petra Prof}{http://www.vision.inst.ac.uk/~pp}{1}
\addauthor{Colin Collaborator}{colin@collaborators.com}{2}

% Enter the institutions
% \addinstitution{Name\\Address}
\addinstitution{
 The Vision Institute\\
 University of Borsetshire\\
 Wimbleham, UK
}
\addinstitution{
 Collaborators, Inc.\\
 123 Park Avenue,\\
 New York, USA
}
